CycleQ: An Efficient Basis for Cyclic Equational Reasoning

We propose a new cyclic proof system for automated, equational reasoning about the behaviour of pure functional programs. The key to the system is the way in which cyclic proof and equational reasoning are mediated by the use of contextual substitution as a cut rule. We show that our system, although simple, already subsumes several of the approaches to implicit induction variously known as "inductionless induction", "rewriting induction", and "proof by consistency". By restricting the form of the traces, we show that global correctness in our system can be verified incrementally, taking advantage of the well-known size-change principle, which leads to an efficient implementation of proof search. Our CycleQ tool, accessible as a GHC plugin, shows promising results on a number of standard benchmarks.

==> redundancies.tex <==
% !TEX root = main.tex

\section{Redundancies}\label{sec:Redundancies}

There are a number of redundancies in the space of possible proofs, accounting for which enables a significantly more performant implementation.

The first redundancy is that a goal equation can be reduced without affecting its provability.
To demonstrate this property, we first introduce an additional inference rule \( \rlnm{Unreduce} \):
\iffalse
\lo{Inference rules are usually named according to the feature / construct that is introduced by the conclusion.
  On this basis, the names \rlnm{Unreduce} and \rlnm{Reduce} should be swapped.}
\ej{As our system is goal directed I think the premises are what is introduced}
\lo{This is reasonable, but it is not applied consistently. E.g.~(FunExt) is the statement ``premises implies conclusion'' i.e.~top down rather then goal directed; also (Start) should probably be (End) if read in a goal-directed manner?}
\fi
\[
  \prftree[r, l]
  {
    \(
    (M \rightarrow_R^* M', N \rightarrow_R^* N')
    % \begin{array}{@{}c}
    %   M \rightarrow_R^* M' \\
    %   N \rightarrow_R^* N'
    % \end{array}
    \)
  }
  {\( \rlnm{Unreduce} \)}
  {\Gamma \vdash M \doteq N : \sigma}
  {\Gamma \vdash M' \doteq N' : \sigma}
\]

%\begin{definition}[Generalised Proof]
By a \defn{generalised proof}, we mean a tuple \( (V,\, E,\ e,\, r) \) following \cref{def:preproof} and \cref{def:proof} but where \( r(v) \) may additional employ the \( \rlnm{Unreduce} \) rule.
%\end{definition}

The unreduce rule is derivable in the sense that it can be directly replaced with applications of other rules without \changed[lo]{affecting} the possible traces.
Suppose there is a derivation of \( \Gamma \vdash M \doteq N : \sigma \).
Then simply consider the extended derivation in \cref{fig:Unreduce is derivable}
\begin{figure*}[ht]
  \[
    \prftree[l]
    {\( \rlnm{Super} \)}
    {
      \prftree[l]
      {\( \rlnm{Reduce} \)}
      {
        \prftree[l]
        {\( \rlnm{Refl} \)}
        {\Gamma \vdash M' \doteq M' : \sigma}
      }
      {\Gamma \vdash M \doteq M' : \sigma}
    }
    {
      \prftree[l]
      {\( \rlnm{Super} \)}
      {
        \prftree[l]
        {\( \rlnm{Reduce} \)}
        {
          \prftree[l]
          {\( \rlnm{Refl} \)}
          {\Gamma \vdash N' \doteq N' : \sigma}
        }
        {\Gamma \vdash N \doteq N' : \sigma}
      }
      {
        \prfsummary
        {\Gamma \vdash M \doteq N : \sigma}
      }
      {\Gamma \vdash M \doteq N' : \sigma}
    }
    {\Gamma \vdash M' \doteq N' : \sigma}
  \]
  \caption{\label{fig:Unreduce is derivable}
    \rlnm{Unreduce} rule is derivable}
\end{figure*}

We will later argue that instances of superposition, where the lemmas are justified by \( \rlnm{Reduce} \), are also redundant.
\lo{Note that in the derivation in \cref{fig:Unreduce is derivable}, for the \rlnm{Super} rule on the right-side, the premise  that is justified by $\rlnm{Reduce}$ (i.e.~$\Gamma \vdash N \doteq N' : \sigma$) is the continuation, not lemma.
  So it follows that this instance of \rlnm{Super} is \textbf{not} redundant (in the sense of \cref{def:redundant Instance of Superposition}).}
\lo{Correction: By commuting the conclusion of the \rlnm{Super}, ethier premise can be considered the lemma.}
However, our proof of this redundancy requires the use of the \( \rlnm{Unreduce} \) rule.
Thus the observation that \( \rlnm{Unreduce} \) can be replaced with this derivation is insufficient as our argument would be circular.

\begin{definition}%[Redundant Instance of Superposition]
  \label{def:redundant Instance of Superposition}
  A \defn{redundant instance of superposition} in a proof \( (V,\, E,\, r,\, e) \) is a vertex \( v_0 \in V \) such that \( r(v_0) \) is an instance of \( \rlnm{Super} \) with lemma \( e(v_1) \) such that \( r(v_1) \) is an instance of \( \rlnm{Refl} \), \( \rlnm{Reduce} \), or \( \rlnm{Super} \).
  We say that \( r(v) \) is redundant for short.
\end{definition}

It is, therefore, necessary to show that \( \rlnm{Unreduce} \) is admissible without such redundant intance of superposition.
First, we shall restrict our attention to a simple class of ``tree-shaped'' proofs.

\begin{definition}%[Tree-Shaped Proofs]
  A \defn{tree-shaped (generalised) proof} is a (generalised) proof \( (V,\, E,\, e,\, r) \) such that the vertices \( V \subseteq \mathbb{N}^* \) are strings of natural numbers  closed under prefix (\( <_\textrm{pre}\)) and where \( E = \{ (v,\, w) \mid \exists i \in \mathbb{N}.\, w = vi \} \).
%\end{definition}

%\begin{definition}%[Breadth-First Order]
  For a tree-shaped proof, we define the \defn{breadth-first order} on vertices, \( v \leq_\textrm{bf} w \), which holds if the string \( v \) is shorter than \( w \) or they have the same length and \( v \leq_\textrm{lex} w \), where \( {\leq_\textrm{lex}} \) is the lexicographical extension of the usual order on natural numbers.
\end{definition}

\cref{lem:unreduce-elim} shows that \( \rlnm{Unreduce} \) commutes with every inference rule in the sense that if any equation is first justified by \( \rlnm{Unreduce} \) and then its premise is subsequently justified by a different rule, it can use that rule immediately and \( \rlnm{Unreduce} \) the premises instead.
Furthermore, this translation respects the progress points of traces in that they also commute with an instance of \( \rlnm{Unreduce} \), and it doesn't introduce redundant instances of superposition (e.g.\ with a \( \rlnm{Reduce} \) vertex as in the aforementioned derivation).

\begin{lemma}\label{lem:unreduce-elim}
  Given a generalised tree-shaped proof \( P = (V,\, E,\, e,\, r) \) with \( v_0 \in V \) such that \( r(v_0) \) is an instance of \( \rlnm{Unreduce} \), then there exists a generalised tree-shaped proof \( P' = (V',\, E',\, e',\, r') \) with \( e'(v_0) = e(v_0) \) but \( r'(v_0) \) is not an instance \( \rlnm{Unreduce} \).
  Furthermore, for all vertices that are not in the subtree rooted at \( v_0 \), i.e. \( w \not>_\textrm{pre} v \),  \( e'(w) = e(w) \) and \( r'(w) = r(w) \).
  And any path segment \( p' = (v_0,\, \dots,\, v_n) \) in \( P' \) such that \( \forall i < n.\, r'(v_i) \) is not an instance of \( \rlnm{Unreduce} \), there is a path segment \( p = (v_0,\, \dots,\, w_m) \) in \( P \) where any trace segment for this path \( t = (M_0,\, \dots,\, M_m) \) can be extended to a trace segment \( t' = (M_0,\, \dots,\, M_n) \) for the path segment \( p' \) such that \( M_n = M_m \) and the trace \( t' \) has a progress point if \( t \) does.
  \begin{proof}
    We proceed by case analysis of the inference rule \( r(v_0) \):
    \begin{itemize}
      \item \( \rlnm{Refl} \) In this case, we have that \( M = N \). By confluence \( M' \) and \( N' \) have a common reduct. And, therefore, we may justify the equation \( \Gamma \vdash M' \doteq N' \) by reduction and reflexivity.
      \item \( \rlnm{FunExt} \) This case is trivial as higher-order terms cannot reduce.
      \item \( \rlnm{Reduce} \) In this case, the equation of \( v_0 \) is \( \Gamma \vdash M'' \doteq N''\) where \( M \rightarrow_R^* M'' \), and \( N \rightarrow_R^* N'' \). By confluence, \( M' \) and \( M'' \) must have a common reduct \( M''' \) and similarly there exists some \( N''' \). Thus we can justify the equation of \( v_0 \) with \( \rlnm{Reduce} \) to the new vertex \( \Gamma \vdash M''' \doteq N''' \) followed by \( \rlnm{Unreduce} \) to the original premise \( \Gamma \vdash M \doteq N \).
      \item \( \rlnm{Super} \) Suppose \( v_0 \) is associated with the equation \( \Gamma \vdash D[M'\sigma] \doteq N' \) with \( N \rightarrow_R N' \). In this case, \( v_1 \) is \( \Gamma \vdash C[L\theta] \doteq N \) with the lemma \( \Delta \vdash L \doteq R \) and the continuation \( \Gamma \vdash C[R\theta] \doteq N \). Furthermore, suppose \( C[L\theta] = D[M\sigma] \) such that \( M \rightarrow M' \in R \). That is, we are considering a deriviation with the following shape:

            \[
              \prftree[r, l]
              {
                \scriptsize
                \(
                \begin{array}{@{}l}
                  M \rightarrow M' \in R \\
                  N \rightarrow_R^* N'   \\
                  D[M\sigma] = C[L\theta]
                \end{array}
                \)
              }
              {\( \rlnm{Unreduce} \)}
              {
                \prftree[l]
                {\(\rlnm{Super}\)}
                {\prfsummary{\Delta \vdash L \doteq R}}
                {\prfsummary{\Gamma \vdash C[R\theta] \doteq N}}
                {\Gamma \vdash C[L\theta] \doteq N}
              }
              {\Gamma \vdash D[M'\sigma] \doteq N'}
            \]

            We consider six cases dependening on the partial-order relationship between \( C \) and \( D \), see \cref{lem:context}.
            In each subcase, \( r'(v_0) \) is \( \rlnm{Super} \):
            \begin{itemize}
              \item If \( C = D \), then pick \( \Gamma \vdash M'\sigma \doteq R\theta \) as the lemma and \( \Gamma \vdash D[R\theta] \doteq N' \) as the continuation. As \( L\theta \rightarrow_R M'\sigma \) and \( N \rightarrow_R^* N' \) both of these intermediate equations follow from \( \rlnm{Unreduce} \) and an original premise.
              \item If they are unrelated, then \( D[M'\sigma] \) also contains the subterm \( L\theta \). Thus we may use the original lemma, leaving the continuation \( \Gamma \vdash D[R\theta/L\theta][M'\sigma] \doteq N' \) where \( D[R\theta/L\theta] \) is the context \( D \) with the subterm \( R\theta \) in the original position of \( L\theta \). This equation is justified by \( \rlnm{Unreduce} \) to \( \Gamma \vdash C[R\theta] \doteq N \), which is also one of the original premises.
              \item Suppose \( D = C \circ E \), i.e. \( D[M'\sigma] = C[E[M'\sigma]] \) and \( E[M\sigma] = L\theta \). We justify \( v_0 \) with \( \rlnm{Super} \) where the lemma is \( \Gamma \vdash E[M'\sigma] \doteq R\theta \) and the continuation is \( \Gamma \vdash C[R\theta] \doteq N' \). By \( \rlnm{Unreduce} \), we can justify the continuation with the original premise \( \Gamma \vdash C[R\theta] \doteq N \). Furthermore, the lemma can be derived from \( \rlnm{Unreduce} \) of \( \Gamma \vdash E[M\sigma] \doteq R\theta \).
              \item Suppose \( C = D \circ E \), i.e. \( M\sigma = E[L\theta] \) and \( D[E[R\theta]] = C[R\theta] \). We justify \( v_0 \) with \( \rlnm{Super} \) where the lemma is \( \Gamma \vdash M'\sigma \doteq E[R\theta] \) and the continuation is \( \Gamma \vdash D[E[R\theta]] \doteq N' \). By \( \rlnm{Unreduce} \), we can justify the continuation with the original premise \( \Gamma \vdash C[R\theta] \doteq N \). Furthermore, the lemma can be derived from \( \rlnm{Unreduce} \) of \( \Gamma \vdash M\sigma \doteq E[R\theta] \).
            \end{itemize}
      \item \( \rlnm{Case} \) In this case, we have that \( v_0 \) is \( \Gamma,\, x : d \vdash M' \doteq N' : \tau \) and \( v_2 \) is \( \Gamma,\, x : d \vdash M \doteq N \) with premsises of the form \( \Gamma,\, \Delta \vdash M\theta \doteq N\theta \). As \( M \rightarrow_R^* M' \) and \( N \rightarrow_R^* N' \) it follows that \( M\theta \rightarrow_R^* M'\theta \) and \( N\theta \rightarrow_R^* N'\theta \) respectively. Thus we can justify \( v_0 \) with \( \rlnm{Case} \) where the intermediate equation \( \Gamma,\, \Delta \vdash M'\theta \doteq N'\theta \) are, in turn, justified by \( \rlnm{Unreduce} \) with the original premise of \( v_1 \).
    \end{itemize}
  \end{proof}
\end{lemma}

We can incrementally apply the aforementioned lemma to eliminate all instances of \( \rlnm{Unreduce} \).

\begin{theorem}[(Admissibility of unreduce)]
  Given a generalised tree-shaped proof \( (V_0,\, E_0,\, e_0,\, r_0) \) with \( v_0 \in V \) such that \( r(v_0) \) is an instance of \( \rlnm{Unreduce} \) but no other vertices are justified by this rule, then there exists a tree-shaped proof \( (V_\infty,\, E_\infty,\, e_\infty,\, r_\infty) \) where there are no vertices such that \( r_\infty(v) \) is an instance of \( \rlnm{Unreduce} \).

  \lo{How do we get to the if part of the theorem?}
  \begin{proof}
    We define a sequence of proofs \( {(P_i)}_{i \in \mathbb{N}} \) and vertices \( {(v_i)}_{i \in \mathbb{N}} \), where \( v_i \in V_i \) by mutual induction:
    \begin{align*}
      P_{i+1} & \defeq \Phi_{v_i}(P_i)                                                                                  \\
      v_{i+1} & \defeq \min_{\textrm{bf}} \{ v \mid v \in V_i,\, r_i(v) \textrm{ is an instance of } \rlnm{Unreduce} \}
    \end{align*}

    Let \( V_0\!\uparrow \) be the subset of vertices from \( P_0 \) from the root up-to \( v_0 \).
    Let \( V_i\!\uparrow \) be the subset of vertices from \( P_i \) in the subtree rooted at \( v_i \) up-to and including vertices justified by \( \rlnm{Unreduce} \), i.e.
    \[ V_i\!\uparrow \;\, \defeq
      \begin{array}{l}
        \{ {v_i}w \in V_i \mid \forall u <_\textrm{pre} w \; .\; r({v_i}u) \textrm{ is not} \\
        \textrm{an instance of } \rlnm{Unreduce} \}.
      \end{array}
    \]
    And, similarly, let \( E_i\!\uparrow \) be thoses edges up-to this vertex. That is, \( E_i\!\uparrow = E_i \cap V_i\!\uparrow \times V_i\!\uparrow \).

    We now define a proof \( (V_\infty,\, E_\infty,\, e_\infty,\, r_\infty) \) as follows.
    Let \( V_\infty = \bigcup_{i \in \mathbb{N}} V_i\!\uparrow \) and \( E_\infty = \bigcup_{i \in \mathbb{N}} E_i\!\uparrow \).
    Let \( r_\infty(v_i) \) to be the rule instance \( r_j(v_i) \) where \( j \) is the smallest index such that \( r_j(v_i) \) is not an instance of \( \rlnm{Unreduce} \) and, similarly, let \( e_\infty(v_i) \) be \( e_j(v_i) \).

    Note that:
    \begin{itemize}
      \item There always exists a \( j \) as \cref{lem:unreduce-elim} only justifies strictly larger vertices by \( \rlnm{Unreduce} \).
      \item Furthermore, \( r_k(v_i) = r_j(v_i) \) and \( e_k(v_i) = e_j(v_i) \) for all \( k > j \) as only the subtree rooted \( v_i \) is modified at each iteration.
    \end{itemize}

    First, we shall show that \( (V_\infty,\, E_\infty,\, e_\infty,\, r_\infty) \) is an ungeneralised preproof.
    Suppose \( v \in V_\infty \), i.e. \( v \) is in the subtree of \( V_i \), for some \( i \), rooted at \( v_i \) and that extends up-to and including the vertices justified by \( \rlnm{Unreduce} \).
    We must show that \( E_\infty \cap \{ v \} \times V_\infty \) includes the premises of \( r_j(v) \) where \( j \) is the smallest index such that \( r_j(v) \) is not an instance of \( \rlnm{Unreduce} \).
    If \( j \) is \( i \), then we are done as \( E_i\!\uparrow \) extends passed \( v \) to include any of its premises.
    Otherwise, \( j > i \) and \( {E_j\!\uparrow} \cap {(\{ v \} \times V_j\!\uparrow)}  \) must include the premises of \( r_j(v) \) as it is not \( \rlnm{Unreduce} \) as required.

    Now we must show \( (V_\infty,\, E_\infty,\, e_\infty,\, r_\infty) \) is also a proof.
    Let \( p \) be a path through this proof.
    To construct a infinitely decreasing trace, we relate this path back to a path through the original proof \( P_0 \).
    The path \( p \) can be decomposed in one of two ways:
    \begin{itemize}
      \item Either it is an infinite sequence of finite path segments \( {(p_i)}_{i \in \mathbb{N}} \), which are each contained within the vertices of a single iteration, \( V_j\!\uparrow \) for some \( j \). Each \( p_i \) is either a finite path segment from \( v_j \) to a vertex justified by \( \rlnm{Unreduce} \) in \( P_j \) (which is the first vertex in the next path segment).
      \item Or it is a finite sequence of similar finite path segments \( {(p_i)}_{i \in I} \) with a final infinite path \( p_k \) (for \( k > \max I \)), which never leaves \( V_j\!\uparrow \) for some \( j \).
    \end{itemize}

    In the latter case, we are done as \( P_j \) is a proof the final infinite path \( p_k \) must have an infinitely progressing trace, which can be extended to the entire proof.

    Now consider the first case.
    Let \( p_i = (v_i,\, \dots,\, w_n) \) be a path contained within a single \( V_j\!\uparrow \).
    We can assume the path starts at \( v_0 \) without loss of generality because \( P_j \) is tree shaped.
    By \cref{lem:unreduce-elim}, there is a path segment \( q = (v_i,\, \dots,\, w_m) \) in \( P_{j - 1} \) where any trace segment for this path \( t = (M_0,\, \dots,\, M_m) \) can be extended to a trace segment \( t' = (M_0,\, \dots,\, M_n) \) for the path segment \( p_i \) such that \( M_n = M_m \) and the trace \( t' \) has a progress point if \( t \) does.
    By induction, a path segment \( q = (q_0,\, \dots,\, q_m ) \) must appear in \( P_0 \) such that \( e_0(q_0) = e_i(v_i) \) and \( e_0(q_m) = e_i(w_n) \).
    As this holds for each path segment, we have an infinite path in \( P_0 \), which must have an infinitely progressing trace that can be extended to a trace for \( p \) as required.
  \end{proof}
\end{theorem}

\begin{corollary}
  \ej{exists a proof where you initially normalise a goal.}
\end{corollary}

It is always possible to convert a infinitary proof, and in particular a cyclic proof, into a tree-shaped proof.
However, the reverse is not true in that there are tree-shaped infinitary proofs that do not have a regular representation.

\begin{lemma}
  For any (generalised) proof \( P = (V,\, E,\, e,\, r) \), there is a (generalised) proof \( P' = (V',\, E',\, e',\, r') \) where the set of proven equations is maintained, i.e. \( \{ e(v) \mid v \in V \} = \{ e'(v) \in v \in V' \} \), but where \( P' \) is tree shaped.
\end{lemma}

It does not necessarily follow, therefore, that the previous theorem holds for cyclic proofs, i.e. a cyclic proof with \( \rlnm{Unreduce} \) can be transformed into a cyclic proof in which it is not used.
However, we conjecture that this also holds and assume so in the following theorems.

\begin{conjecture}\label{conj:unreduce-elim}
  Given a generalised cyclic proof \( (V,\, E,\, e,\, r)\), there is an ungeneralised cyclic proof \( (V',\, E',\, e',\, r') \) where there are no redundant instances of superposition that do not appear in the original.
\end{conjecture}

The second redundancy is that superposition need only be performed with a subset of available lemmas.
As superposition is used as a matching function to create cycles, it is particularly important that fewer lemmas are trialled because cycles are costly to verify, see \cref{sec:size-change}.

\begin{definition}%[Redundancy Number]
  Let \( v \) be a vertex from a cyclic proof \( (V,\, E,\, r,\, e) \).
  The \emph{transitive lemmas} of a vertex \( v \), denoted \( L(v) \), is a set of vertices defined as the union of \( L_i \) where:
  \begin{align*}
    L_0       & \defeq \{ v \}                                                                      \\
    L_{i + 1} & \defeq \{ v' \mid v \in L_i,\, (v,\, v') \in E,\, r(v) \textrm{ is an instance of } \\
              & \quad\quad\rlnm{Super} \textrm{ with premise } e(v') \}
  \end{align*}

  Then the \defn{redundancy number} of \( v \), denoted \( n(v) \), is defined as the number of redundant transitive lemmas, \(    \lvert \{ v \in L(v) \mid r(v) \textrm{ is redundant}\} \rvert  \).
  And the redundancy number of the proof itself as the sum of the redundancy number for each vertex \( \sum_{v \in V} n(v) \).
\end{definition}

\begin{theorem}[(Redundancy of superposition)]
  \changed[lo]{Assuming \cref{conj:unreduce-elim}}, for any cyclic proof, there exists a cyclic proof \( (V',\, E',\, r',\, e') \) with the same set of equations but where there are no redundant instances of superposition.
  % \begin{proof}
  %   The proof is by induction on the number of redundant instances \( n \), which is necessarily finite in cyclic proofs.
  %   \begin{itemize}
  %     \item If \( n = 0 \), then we are clearly done.
  %     \item Otherwise, suppose the theorem holds for all proofs with \( n - 1 \) instances. Let us consider an instance that appears in the proof by case analysis of \( r(v_1) \):
  %     \begin{itemize}
  %       \item \( \rlnm{Refl} \) In this case, the conclusion \( v_0 \) and the continuation \( v_2 \) have the same equation and we can use \( r(v_2) \) to justify \( r'(v_0) \). Any infinite path in the resulting graph trivially corresponds to a path in the original graph.
  %       \item \( \rlnm{Reduce} \) Suppose the conlusion equation is \( \Gamma \vdash C[M\theta] \doteq R \), the lemma is \( \Delta \vdash M \doteq N \) justified with \( \rlnm{Reduce} \) of \( \Delta \vdash M' \doteq N' \) such that \( M \rightarrow_R^* M' \) and \( N \rightarrow_R^* N' \), and the continuation is \( \Gamma \vdash C[N\theta] \doteq R \). Let \( r'(v_0) \) be \( \rlnm{Reduce} \) with the premise \( \Gamma \vdash C[M'\theta] \doteq R \), which, in turn, is justified by \( \rlnm{Super} \) with the lemma \( \Delta \vdash M' \doteq N' \) and continuation \( \Gamma \vdash C[N'\theta] \doteq R \). The continuation can be justified by \( \rlnm{Unreduce} \) with the premise \( \Gamma \vdash C[N\theta] \doteq R \).
  %       \item \( \rlnm{Super} \) 
  %     \end{itemize}
  %   \end{itemize}
  % \end{proof}
\end{theorem}


==> size-change.tex <==
% !TEX root = main.tex
\section{Verifying cycles}\label{sec:size-change}

The general global correctness condition is likely to be undecidable as there are countably many terms that could consistute a trace.
If we restrict our attention to a subset of terms such as those that appear in the equation, however, it becomes decidable assuming the term order is also decidable.
A particular instance of this was first shown by reduction to B{\"u}chi automata in the original work on cyclic proofs~\cite{brotherston2005cyclic}.
Informally, two \(\omega \)-regular languages are extracted from a preproof: the path language and the trace language.
It can then be checked whether the path language is included in the trace language, i.e.\ every path has an infinitely progressing trace.

Unfortunately, checking the inclusion of B{\"u}chi automata is doubly exponential in the number of vertices.
This procedure, therefore, becomes intractable if several candidates proofs, the majority of which will be invalid, need to be checked throughout the proof search.
In the Cyclist theorem prover, soundness checking could take up to 44\% of the proof time~\cite{stratulat2019efficient}.

For our implementation, which uses the substructural order, we restricted our attention to variables.
In this setting, we can observe that the global correctness condition is equivalent to the termination of a program.
Therefore, we can adapt the size-change graph approach to verify program termination~\cite{lee2001size}.
The advantage of this approach is that it can be encoded directly in the proof graph making it more amenable to incremental computation.
The workload can be performed as each node is uncovered, with the payoff being that the soundness condition is represented explicitly.
And thus, no unsound proofs need to be checked.

\begin{definition}%[Size-Change Graphs]
  Let \( e(v) = \Gamma \vdash \phi \) and \( e(v') = \Gamma' \vdash \phi'  \) be two vertices in a preproof \( (V,\, E,\, e,\, r) \).
  A \defn{size-change graph (SCG)} between from \( v \) to \( v' \), written \( G : v \rightarrow v' \), is a bipartite graph with vertex sets formed from the variables of \( \Gamma \) and \( \Gamma' \) respectively.
  For two variables, we denote edges as \( x \rightarrow y \) or \( x \searrow y \) if it is decreasing (i.e.\ a possible progress point).
\end{definition}

\begin{definition}[(The SCG of an edge)]
  Let \( (V,\ E,\, e,\, r) \) be a preproof.
  We associate a size change graph \( G_{(v,\, v')} : v \rightarrow v' \) to edge \( (v,\, v') \in E \) as follows:

  \begin{itemize}
    \item If \( r(v) \) is an instance of \rlnm{Super} with substitution \( \theta \) and \( v' \) is the lemma, then there is a non-decreasing edge \( x \rightarrow y \in G_{(v,\, v')} \) if \( x = \theta(y) \).
    \item If \( r(v) \) is an instance of \rlnm{Case} and the expression being analsysed is a variable \( x \), then there is a decreasing edge \(x \searrow y \) for each fresh variable \( y \) introduced into \( v' \) and a non-decreasing edge \( z \rightarrow z \) for all variables including \( x \).
    \item Otherwise, the SCG is simply the identity: \( z \rightarrow z \) for all variables found in both environments.
  \end{itemize}
\end{definition}

Over this domain, two \( \omega \)-regular languages are considered: the flow language of possible call sequence, and the descending language of decreasing calls, which must be included in the former.
For the variable based traces used in our proof system, the SCT problem and the existence of an infinitely progressing trace are clearly equivalent.
This is more than a coincidence; the Curry-Howard correspondence provides an interpretation of preproofs as well-typed programs and proofs proper as a terminating subset.

However, the abstract domain of size-change graphs also enables a compositional approach aside from the reduction to B{\"u}chi automata.
Which, as far as we are aware, has not been previously employed for verifying cyclic preproofs.

\begin{definition}[(Composition of size-change graphs)]
  Given two size-change graphs \( G : v \rightarrow v' \) and \( G' : v' \rightarrow v'' \), then there is a size-change graph \( G' \circ G : v \rightarrow v'' \) defined by the following set of edges.
  There is an edge \( x \rightarrow z \) whenever there exists a variable \( y \) in the type environment of \( v' \) and edges \( x \rightarrow y \in G \) and \( y \rightarrow y \in G' \). It is decreasing if either edge is decreasing.
\end{definition}

% Notice that 
%   For a given preproof, there is a category of vertices with size-change graphs as morphisms.
% \end{lemma}

\begin{definition}%[Closure of a Preproof]
  The \defn{closure of a preproof} \( P = (V,\, E,\, e,\, r) \) is a set of size-change graphs, \( \mathrm{cl}(P) \), such that
  \begin{itemize}
    \item For each edge \( (v,\, v') \in E \), \( G_{(v,\, v')} \in \mathrm{cl}(P) \)
    \item If  \( G : v \rightarrow v' \in \mathrm{cl}(P) \) and \( G' : v' \rightarrow v'' \in \mathrm{cl}(P) \), then \( G' \circ G \in \mathrm{cl}(P) \)
  \end{itemize}
\end{definition}

\begin{lemma}
  For every path segment from \( v \) to \( v' \) in a preproof \( P = (V,\ E,\, e,\, r) \) there is a size-change graph \( G : v \rightarrow v' \in \mathrm{cl}(P) \).
  \begin{proof}
    
  \end{proof}
\end{lemma}

\begin{lemma}
  Let \( P = (V,\ E,\, e,\, r) \) be a preproof.
  If \( G : v \rightarrow v' \in \mathrm{cl}(P) \) is the size-change graph for a particular path segment \( p = (v,\, \dots,\, v') \) and it has a decreasing edge \( x \searrow y \), then there is a trace segment of the form \( (x,\, \dots,\, y) \) with a progress point for this path segment.
  \begin{proof}
    We proceed by induction on the length of \( p \).
    \begin{itemize}
      \item If \(\lvert p \rvert \leq 0 \), then there is nothing to show as there is no size-change graph.
      \item Let \( p = (v,\, \dots,\, v',\, v'') \) and suppose the property holds of \( p = (v,\, \dots,\, v') \). That is, if the size-change graph \( G : v \rightarrow v' \in \mathrm{cl}(P) \) has a decreasing edge \( x \searrow y \), then there is a trace segment of the form \( (x,\, \dots,\, y) \) with a progress point for this path segment. Let \( G' : v' \rightarrow v'' \) be the size-change graph of the final edge in this path segment. Then the size-change graph \( G' \circ G :  v \rightarrow v'' \in \mathrm{cl}(P) \) corresponds to the path segment \( p \). There are two cases where this size-change graph has a decreasing edge:
      \begin{itemize}
        \item \( G' \) has a decreasing edge \( z \searrow y \) and either \( x \searrow z \) or \( x \rightarrow z \) appear in \( G \). In this case, their composition has a decreasing edge 
      \end{itemize} if and only if, \( G' \) has a decreasing edge and ... or \( G \) does. In the latter case 
    \end{itemize}
  \end{proof}
\end{lemma}

\begin{corollary}
  Let \( P = (V,\ E,\, e,\, r) \) be a preproof.
  If \( G : v \rightarrow v' \in \mathrm{cl}(P) \) is the size-change graph for a cycle \( (v,\, \dots,\, v) \) and it has a decreasing edge \( x \searrow x \), then the cycling path has an infinitely progressing trace.
  \begin{proof}
    By the previous lemma, there is a trace segment \( (x,\, \dots,\, x) \) for this cycle.
    Clearly, this can be extended to an trace for the cycling path as the start and end trace elements align.
  \end{proof}
\end{corollary}

\begin{theorem}
  A cyclic preproof \( P = (V,\, E,\, e,\, r) \) is a proof if, and only if, every \( G : v \rightarrow v \in \mathrm{cl}(P) \) such that \( G = G \circ G \) has a decreasing edge \( x \searrow x \) for some variable \( x \).
  \begin{proof}
    Let \( {(v_i)}_{i \in \mathbb{N}} \) be a path through \( P \).
    By the lasso property of \( \omega \)-regular languages, this path must ultimately form a cycle.
    Thus there is some path segment \( (v,\,\ \dots,\, v) \).
    In which case, there is a corresponding size-change graph \( G : v \rightarrow v \in \mathrm{cl}(P) \) such that \( G = G \circ G \).
    By assumption it has a decreasing edge \( x \searrow x \) for some variable \( x \).
    And so the trace that is eventually \( x \) is infinitely progressing as required.
  \end{proof}
\end{theorem}
